$k$-Universality of Regular Languages Revisited

A subsequence of a word $w$ is a word $u$ such that $u = w[i_1] w[i_2] \cdots w[i_k]$, for some set of indices $1 \leq i_1 < i_2 < \dots < i_k \leq \vert w \vert$. A word $w$ is \emph{$k$-subsequence universal} over an alphabet $\Sigma$ if every word over $\Sigma$ up to length $k$ appears in $w$ as a subsequence. In this paper, we revisit the problem $k$-ESU of deciding, for a given integer $k$, whether a regular language, given either as nondeterministic finite automaton or as a regular expression, contains a $k$-universal word. [Adamson et al., ISAAC 2023] showed that this problem is NP-hard, even in the case when $k=1$, and an FPT algorithm w.r.t. the size of the input alphabet was given. In this paper, we improve the aforementioned algorithmic result and complete the analysis of this problem w.r.t. other parameters. That is, we propose a more efficient FPT algorithm for $k$-ESU, with respect to the size of the input alphabet, and propose new FPT algorithms for this problem w.r.t.~the number of states of the input automaton and the length of the input regular expression. We also discuss corresponding lower bounds. Our results significantly improve the understanding of this problem.

==> conclusion.tex <==
\todoah{update conclusion when main part is finished}
In this paper, we extended the study of $k$-subsequence universality to subregular languages and contextual grammars. Explicitly, we show that both the $k$-ESU and $k$-USU problems are trivial for monoidal, combinational, finite definite, and symmetric definite languages. The $k$-ESU problem is NP-hard for nilpotent, prefix-closed, suffix closed, left-sided-comet, right-sided-comet, two-sided-comet, ordered, and circular languages.
%Further, the $k$-ESU problem can be decided in polynomial time for contextual grammars. For internal contextual grammars we conjecture NP-hardness since the decision relays on detecting cycles or successively applicable selectors. A reduction for this problem remains open for further research.\looseness=-1

There are two natural directions to peruse following the work. First is improving the parametrised algorithms given in \cite{regunivpaper} for certain classes of subregular languages. Notably, it seems likely that ordered languages may yield an improved fixed parameter algorithm following the same approaches outlined in this paper with the parametrised algorithm of \cite{regunivpaper}. The second direction is to look are further classes of languages, perhaps most naturally those regular languages where the input is given by a regular expression. While regular expression can encode the same set of languages as NFAs, the representation requires significantly more space in general, with the encoding used in the hardness reduction requiring exponentially more space to be represented as a regular expression versus the automaton based representation. Therefore, it is reasonable to assume that we may be able to find more efficient algorithms relative to the input size for solving the $k$-ESU and $k$-USU problems in these languages.\looseness=-1

==> contextual.tex <==
\todoah{$\downarrow$ maybe delete this section}

We now introduce contextual grammars as first defined by Marcus \cite{marcus1969contextual} (also referred to as \emph{external contextual grammars} in the literature).
As defined in \cite{marcus1969contextual}, a pair $(u,v) \in \Sigma^* \times \Sigma^*$ is called a \emph{context} on $\Sigma$ and $\mathcal{C}$ denotes the set of contexts.

\begin{definition}
	Given a finite language $L_1 \subset \Sigma^*$ and a finite set $\mathcal{C}$ of contexts in $\Sigma$. The tuple $G= (\Sigma, L_1, \mathcal{C})$ is a \emph{contextual grammar}. The language generated by $G$ is said to be a \emph{contextual language} and denoted by $L(G)$ and is defined as the smallest language $L\subseteq \Sigma^*$ such that 
	\begin{enumerate}
		\item $L_1 \subseteq L$, and
		\item if $x \in L$ and $(u,v) \in \mathcal{C}$ then $uxv \in L$.
	\end{enumerate}
\end{definition}

\begin{proposition}
	Let $G=(\Sigma, L_1, \mathcal{C})$ be a contextual grammar. If $L_1 \neq \emptyset$ and there exists $(u,v) \in \mathcal{C}$ with $\al(u) = \Sigma$ or $\al(v) = \Sigma$ then $L(G)$ is $k$-$\exists$-universal for all $k \in \N$.
\end{proposition}
\begin{proof}
	Let $x \in L_1$ and w.l.o.g.~let $\al(u) = \Sigma$. Since $G$ is a contextual grammar, we have $u^n x v^n \in L(G)$ for all $n \in \N$. Further, $\iota(u^n x v^n) \geq n$, i.e., $L(G)$ is $k$-$\exists$-universal for all $k \in \N$.\qed
\end{proof}
\todo[inline]{Prop28 is pointless since Prop29 generalizes it}
\begin{proposition}
	Let $G=(\Sigma, L_1, \mathcal{C})$ be a contextual grammar. If $L_1 \neq \emptyset$ and there exists a sequence $(u_1,v_1), \ldots, (u_n, v_n) \in \mathcal{C}$ for some $n \in \N$ with $\bigcup_{i \in [n]}\al(u_i) = \Sigma$ or $\bigcup_{i \in [n]} \al(v_i) = \Sigma$ then $L(G)$ is $k$-$\exists$-universal for all $k \in \N$.
\end{proposition}
\begin{proof}
	Let $x \in L_1$ and w.l.o.g.~let there exist some $n \in \N$ and a sequence $(u_1,v_1), \ldots, (u_n, v_n) \in \mathcal{C}$ such that $\bigcup_{i \in [n]}\al(u_i) = \Sigma$. By definition we get that $(u_1 \cdots u_n)^\ell x (v_1 \cdots v_n)^\ell \in L(G)$ for all $\ell \in \N$. Thus, $\iota((u_1 \cdots u_n)^\ell x (v_1 \cdots v_n)^\ell) \geq \ell$, i.e., $L(G)$ is $k$-$\exists$-universal for all $k\in \N$. \qed
\end{proof}

\begin{proposition}
	Let $G=(\Sigma, L_1, \mathcal{C})$ be a contextual grammar. If $L_1 \neq \emptyset$ and for all sequences $(u_1,v_1), \ldots, (u_n, v_n) \in \mathcal{C}$ for $n \in \N$ we have $\bigcup_{i \in [n]}\al(u_i) \subset \Sigma$ and $\bigcup_{i \in [n]} \al(v_i) \subset \Sigma$ then there exists a $k \in \N$ such that $L(G)$ is not $k$-$\exists$-universal.
\end{proposition}
\begin{proof}
	Since $L_1 \neq \emptyset$, there exists $x \in L_1$.
	Let $\iota(L_1) = \max_{x \in L_1} \iota(L_1)$ denote the maximal universality in $L_1$ (there exists such a value since $L_1$ is finite). Then, we obtain for any $w = uxv \in L(G)$ for $u = \prod_{i=1}^n u_i$, $v = \prod_{i=1}^n v_i$ with $n \in\N$ and $(u_i,v_i) \in \mathcal{C}$ for $i\in[n]$ and $x \in L(G)$  that $\iota(w) \leq \iota(L_1) + 2$ since there might exist a prefix $p$ and a suffix $s$ of $x$ not overlapping with $p$ such that $\bigcup_{i \in [n]}\al(u_i)  \cup \al(p)= \Sigma$ and $\bigcup_{i \in [n]} \al(v_i) \cup \al(s)= \Sigma$. Thus, we can conclude that $L(G)$ is not $k$-$\exists$-universal for all $k > \max(1,\iota(L_1)) + 2$.\qed
\end{proof}
%\todo[inline]{3. Why is $\iota(w)\leq max(1,\iota(L_1)$? I don't see any possibility that $\iota(w)=3$ if $iota(L_1)=0$ (the first arch of $w$ ends somewhere in $xv$ and $xv$ is not $2-universal$).}
\begin{corollary}\label{contextual:kESUforallk}
	Let $G=(\Sigma, L_1, \mathcal{C})$ be a contextual grammar. The following statements are equivalent:
	\begin{enumerate}
		\item $L_1 \neq \emptyset$ and there exists a sequence $(u_1,v_1), \ldots, (u_n, v_n) \in \mathcal{C}$ for some $n \in \N$ with $\bigcup_{i \in [n]}\al(u_i) = \Sigma$ or $\bigcup_{i \in [n]} \al(v_i) = \Sigma$, and
		\item $L(G)$ is $k$-$\exists$-universal for all $k \in \N$.
	\end{enumerate}  
\end{corollary}

\begin{corollary}
%	\todoah{$\downarrow$ this proposition is not correct, the problem falls back on deciding the $k$-universality of $L_1$ so this is NP-hard too :(}
	Let $L_1\neq\emptyset$. For all $k\in \N$ and contextual languages represented by their contextual grammar $(\Sigma,L_1,\mathcal{C})$ the problem $k$-ESU is NP-hard.
\end{corollary}
\begin{proof}
	Since $L_1$ is a finite language, the problem of determining the $k$-universality of words in $L(G)$ falls back to determine the $k$-, $(k-1)-$, or $k-2$-universality of words in $L_1$ which is NP-hard by \cite{regunivpaper}.\qed
\end{proof}
%\begin{proof}
%	%	Let $\mathcal{C}[1] = \\{u \mid (u,v) \in \mathcal C\}$ and $\mathcal{C}[2] = \\{v \mid (u,v) \in \mathcal C\}$.
%			Using a union-find data structure with union-by-size and path compression, we can compute $U= \bigcup_{i \in |\mathcal{C}|} \{u_i \mid (u_i,v_i) \in \mathcal{C}\}$ and $V= \bigcup_{i \in |\mathcal{C}|} \{v_i \mid (u_i,v_i) \in \mathcal{C}\}$ both in $O(1)$ time. Now using $\sigma$ find operations in $O(\sigma \log(|\mathcal{C}|))$ we can check whether $\Sigma = \al(U)$ or $\Sigma = \al(V)$ holds. If so, we positively decide $k$-ESU for all $k \in \N$ according to Corollary~\ref{contextual:kESUforallk}. If not, then we compute the largest universality index of $L_1$ in $O(|L_1|)$ time. Let $W \subseteq L_1$ be the set of words with the largest universality index and $W' \subseteq L_1$ the set of words with the second largest universality index. 
%			Now for all $w \in W$ we check whether $\Sigma \setminus \al(U) \subset \al(\inner_1(w))$ or $\Sigma \setminus \al(U) \subset \al(r(w))$ hold. If both is true, then we negatively decide $k$-ESU for all $k > \iota(w) +2$ and positively otherwise. If only one of them holds then we negatively decide $k$-ESU for all $k > \iota(w) +1$ and positively otherwise. Otherwise, we consider words $w' \in W'$: If $\iota(w') = \iota(w) -1$ then we check whether $\Sigma \setminus \al(U) \subset \al(\inner_1(w'))$ and $\Sigma \setminus \al(U) \subset \al(r(w'))$. If so, then we negatively decide $k$-ESU for all $k > \iota(w) +1$ and positively otherwise. If not, then we decide negatively $k$-ESU for all $k > \iota(w) +1$ and positively otherwise. This whole decision procedure relies on several computations of the arch factorisation and can be computed in $O(|W|+|W'|)$ time which can be estimated by $O(|L_1|)$ time.\looseness=-1
%			%	In runtime $O(|\mathcal{C}|!)$ we can check whether there exists a sequence $(u_1,v_1), \ldots, (u_n, v_n) \in \mathcal{C}$ for some $n \in \N$ with $\bigcup_{i \in [n]}\al(u_i) = \Sigma$ or $\bigcup_{i \in [n]} \al(v_i) = \Sigma$. If so, then we positively decide $k$-ESU for all $k \in \N$ according to Corollary~\ref{contextual:kESUforallk}. If not, then we compute the largest universality index of $L_1$ in $O(|L_1|)$ time. Let $w \in L_1$ be the word with the largest universality. If there exists $(u,v) \in \mathcal{C}^*$ such that $\iota(uwv) = \iota(w) +2$ then negatively decide $k$-ESU for all $k > \iota(w) +2$ and positively otherwise.  Otherwise, if there exists $(u,v) \in \mathcal{C}^*$ such that $\iota(uwv) = \iota(w) +1$ then negatively decide $k$-ESU for all $k > \iota(w) +1$ and positively otherwise. If $\iota(uwv) = \iota(w)$ for all $(u,v) \in \mathcal{C}^*$ then negatively decide $k$-ESU for all $k > \iota(w)$ and positively otherwise. The existence of such $u$ and $v$ can be checked in $O(|\mathcal{C}|!)$. Thus, we have a total runtime of $O(|\mathcal{C}|!)$.
%		\end{proof}
%		\todo[inline]{The complexity is not correct if $\mathcal C$ is large compared to $L_1$. We need some time to compute the alphabets of $U$ and $V$. Also, checking whether $L_1$ has $(k-1)$- or $(k-2)$-universal words is NP-hard.}
		
		\subsection{Internal Contextual Grammars}
		
		Subsequent studies on contextual grammars further extended the definition from \cite{marcus1969contextual} to, e.g., deterministic, parallel, normal and modular contextual grammars (see \cite{Ehrenfeucht1997} for a survey). We will focus on the notion of internal contextual grammars that were firstly introduces by Ilie in \cite{ILIE199733}.\looseness=-1
		
		\begin{definition}
			For $n \in \N$, an \emph{internal contextual grammar} (ICG) is a tuple $G = (\Sigma, A, (S_1,C_1), \ldots, (S_n,C_n))$  with an alphabet $\Sigma$, a finite set of \emph{axioms} $A \subseteq \Sigma^*$, sets of \emph{selectors} $S_i \in \Sigma^*$ for $i \in [n]$ and a set of \emph{contexts} $C_i \in \Sigma^* \times \Sigma^*$ with finite $C_i$ for $i \in [n]$.
		\end{definition}
		
		\begin{definition}
			A derivation step in an ICG $G = (\Sigma, A, (S_1,C_1), \ldots, (S_n,C_n))$ for $n \in \N$ and $x,y \in \Sigma^*$ is defined by $x \Rightarrow y$ iff $x = x_1 x_2 x_3, y = x_1 u x_2 v x_3$, where $x _2 \in S_i$ and $(u,v) \in C_i$ for some $i \in [n]$. Further, we write $\alpha \Rightarrow^* w$ for $\alpha \in A$ and $w \in \Sigma^*$ if there exists a finite sequence of derivations transforming $\alpha$ into $w$.
			
			The language generated by an ICG $G=(\Sigma, A, (S_1,C_1), \ldots, (S_n,C_n))$ is $L(G) = \{w \in \Sigma^* \mid \exists \alpha \in A \colon \alpha \Rightarrow^* w\}$.
		\end{definition}
		
		Note that the language generated by an ICG $G =(\Sigma, A, (S_1,C_1), \ldots, (S_n,C_n))$ is empty if $A \cap \bigcup_{i \in [n]} S_i = \emptyset$ since there is no derivation applicable from any axiom. 
		
		\begin{proposition}\label{internalcontextual:kESUforallk}
			Let $G=(\Sigma, A, (S_1,C_1), \ldots, (S_n,C_n))$ be an internal contextual grammar. If there exist an $i \in [n]$ s.t. $\alpha \in A \cap S_i$, $(u_i,v_i) \in C_i$ and $\iota(u_i) \geq 1$ or $\iota(v_i) \geq 1$ then $L(G)$ is $k$-$\exists$-universal for all $k \in \N$.
		\end{proposition}
		\begin{proof}
			By definition, $\alpha \Rightarrow^* (u_i)^k \alpha (v_i)^k$ for any $k\in\mathbb N$. Thus, we can conclude that there exists a $k$-universal word for every $k\in \N$ if $u_i$ or $v_i$ do contain every letter at least once.\qed
		\end{proof}
		
		Notice, that we cannot easily give the reverse implication of Proposition~\ref{internalcontextual:kESUforallk} because of two reasons. First, there might be circles in the selector-context-pairs that need to be detected. Consider for example the ICG $G = (\{\ta, \tb, \tc\}, \{\ta\}, (\ta, (\tb,$ $\tb)), (\tb, (\ta,\ta)),(\ta, (\tc,\tc)))$. Here we have the circle that any $\ta$ can be surrounded by $\tb$ and v.v.~as well as getting $\tc$ from $\ta$. Thus, starting with $\ta$ we can produce $k$-universal words for any $k \in \N$ since from $\ta$ we can generate any other letter and also produce even more $\ta$. Second, we need to tackle the problem of selectors that may not be applicable on the set $A$ but later when performed a series of productions, e.g., $G = (\{\ta, \tb,\tc\}, \{\ta\}, (\ta, (\ta\tb,\ta\tb)),(\tb\ta, (\tc,\tc)))$. Here the second selector-context-pair is not applicable on $A$ but there exist derivations such that it gets applicable in further derivation steps, i.e., we need to search for the point where such selectors might get applicable.
\todo[inline]{We should work on the inverse implication!}
%		\begin{proposition}\label{internalcontextual:kESUforallkeq}
%			\todoah{this is still under construction, currently incorrect}
%			Let $G=(\Sigma, A, (S_1,C_1), \ldots, (S_n,C_n))$ be an internal contextual grammar. The following statements are equivalent:
%			\begin{enumerate}
%				\item there exist an $i \in [n]$ s.t. $\alpha_i \in A \cap \bigcup_{i \in [n]} S_i$ and a sequence $(u_1,v_1), \ldots, (u_n, v_n) \in \mathcal{C}$ for some $n \in \N$ with $\bigcup_{i \in [n]}\al(u_i) = \Sigma$ or $\bigcup_{i \in [n]} \al(v_i) = \Sigma$, and
%				\item $L(G)$ is $k$-$\exists$-universal for all $k \in \N$.
%			\end{enumerate}  
%		\end{proposition}
		
%		{\color{red}In \cite{ILIE199733}, the author also introduced \emph{local ICG's} where contexts are only allowed to be placed inside of or adjacent to a previous context. Thus, derivations are restricted to certain forms.
%		
%		\begin{definition}
%			Let $z \Rightarrow x$ with $z = z_1 z_2 z_3 \in \Sigma^*$ and $z_2 \in S_i, (u,v) \in C_i$ and $x = z_1 u  z_2 v z_3$ for $i \in \N$ be a derivation. The derivation $x \Rightarrow y$ is \emph{local} w.r.t.~the derivation $z \Rightarrow x$ ($z \Rightarrow x \Rightarrow_{loc} y$) iff
%			\begin{enumerate}
%				\item $u = u' u'', v = v' v''$ for $u',u'',v',v'' \in \Sigma^*$,
%				\item $x = x_1 x_2 x_3$ with $x_1 = z_1 u', x_2 = u'' z_2 v', x_3 = v'' z_3$, 
%				\item $x_2 \in S_j, (w,t) \in C_j$ for some $j \in [n]$, and 
%				\item $y = x_1 w x_2 t x_3$. 
%			\end{enumerate}
%			The language generated by an ICG $G=(\Sigma, A, (S_1,C_1), \ldots, (S_n,C_n))$ by local derivations is $L_{loc} (G) = \{w \in \Sigma^* \mid \exists \alpha \in A \colon \alpha \Rightarrow_{loc}^* w\}$.
%		\end{definition}}

==> countingandranking.tex <==
\label{sec:counting}


In this section we discuss the problems of counting and ranking efficiently $k$-universal words from a regular language, given as a DFA, or $k$-universal paths in the case when the respective language is given as an NFA. Note, that there is a one-to-one correspondence between paths and words in the case of DFAs, so, for the sake of simplicity, from now on we will simply talk about counting and ranking paths accepted by the finite automata we are given as input.

Here, we define the problem of \emph{counting} and \emph{ranking} problems, for a given automaton $\mathcal{A}$, and universality index $k$. The counting problem is defined as the problem of determining the number of $k$-universal words accepted by $\mathcal{A}$, equivalent to determining the size of $\Univ_{L(\mathcal{A}), k}$. For a given length $m \in \mathbb{N}$, the problem of counting the number of $k$-universal words of length exactly (respectively, at most) $m$ is the problem of determining the size of $\Univ_{\mathcal{A}_m, k}$ (respectively $\Univ_{\mathcal{A}_{\leq m}, k}$. The \emph{rank} of a word $w \in \mathcal{A}_n$ is the number of $k$-universal words accepted by $\mathcal{A}$ that are smaller than $w$, i.e. the size of  $\{v < w \mid v \in \Univ_{L(\mathcal{A}), k} \} $. For a given length $m$, the \emph{rank} of $w$ within the set of $k$-universal words of length exactly (respectively, at most) $m$ is the problem of determining the size of the set $\vert \{ v < w \mid v \in \Univ_{\mathcal{A}_m, k} \} \vert$ (respectively, $\vert \{ v < w \mid v \in \Univ_{\mathcal{A}_{\leq m}, k} \} \vert$).

Recall that we are operating on a DFA or NFA $\mathcal{A}$ with $n$ states and an alphabet of size $\sigma > 1$ (the case $\sigma=1$ is trivial). We are also given as input the natural numbers $k$ and $m$ in binary representation: we are interested in counting (ranking) the $k$-universal words of length $m$ contained in $L(\mathcal{A})$. It is important to know that these problems are only interesting for $k\leq m/\sigma$; otherwise, there are no $m$-length $k$-universal words. However, an additional difficulty related to this problem, compared to the case of the decision problems discussed in Section \ref{npc}, is that we need to do arithmetics with large numbers. In general, if $M$ is an upper bound on the value of the numbers that we need to process and $\omega$ is the size of the memory word of our model, then each arithmetic operation requires at most $O(\frac{ \log M }{\omega})$ time to complete. In the cases we approach here, $M\leq (n\sigma)^{m+1}$ (a crude upper bound on the total number of paths of length at most $m$ in $\mathcal{A}$), so each arithmetic operation requires at most $O(\frac{(m+1) \log (n\sigma) }{\omega})$, that is $O^*(m)$ time. 

This section is laid out as follows. First, we consider the problems of counting the number of $k$-universal accepting  paths of the finite automaton $\mathcal{A}$. For a given $m \in \N$ this is split into two cases, counting  the number of $k$-universal accepting paths of $\mathcal{A}$ of length exactly $m$, and counting the number of $k$-universal accepting paths of $\mathcal{A}$ of length at most $m$. We show that both can be computed in $O^*(m^2 n^2 k 2^{\sigma})$ time.
% in $O(m^2 n^2 k \sigma 2^{\sigma})$ time.
Additionally, we show that the number of $k$-universal accepting paths of $\mathcal{A}$ can be computed in 
$O^*(n^4 k^2 2^{\sigma})$ time.
% $O(n^4 k^2 \sigma^2 2^{\sigma})$ time.

We extend our counting results to the ranking setting, showing that a path $\pi$ (respectively, word $w$) can be ranked within the set of $k$-universal paths (respectively, words) of length exactly $m$ accepted by the NFA (respectively, DFA) ${\mathcal A}$ in 
% $O(m^2 n^2 k \sigma 2^{\sigma})$ 
$O^*(m^2 n^2 k 2^{\sigma})$ 
% time, of length at most $m$ in $O(m^2 n^2 k \sigma 2^{\sigma})$ time, and of any length in $O(n^4 k^2 \sigma^2 2^{\sigma})$ time.
time, of length at most $m$ in $O^*(m^2 n^2 k 2^{\sigma})$ time, and of any length in $O^*(n^4 k^2 2^{\sigma})$ time.
% Note that these match the counting results, and indeed the counting results provide a weak lower bound to the ranking problem, as the total number of $k$-universal words accepted by $\mathcal{A}$ can be counted by computing the rank of the lexicographically largest word.
% Therefore, the time complexity of any ranking algorithm must be greater than or equal to the complexity of counting the number of $k$-universal words.

The main tool used in this section is the $n \times (m + 1) \times k \times 2^{\sigma}$ size table $T$, which we refer to as the \emph{path table of length $m$} for a given $m\in\N_0$.
% The high level idea for a deterministic finite automaton $\mathcal{A}$ is to construct an $n \times m \times k \times 2^{\sigma}$ size table $T$, which we refer to as the \emph{path table}.
Each entry in the table $T$ is indexed by a state $q \in Q$, a length $\ell \in [0, m]$, the number of arches $c \in [0, k-1]$, and a subset of symbols $\mathcal{R} \subset \Sigma$. The entry $T[q, \ell, c, \mathcal{R}]$ contains the number of $\ell$-length paths starting at the state $q_0$ and ending in the state $q$ such that the words induced by the paths contain each $c$ arches, and the alphabet of the rest  is $\mathcal{R}$. Thus,
in the context of the arch factorisation, we are interested in all words belonging to paths in $\mathcal{A}$ which are {\em not yet} $k$-universal.
Formally, we have $T[q, \ell, c, \mathcal{R}] = \sum_{w \in \Sigma^\ell, \letters(\r(w)) = \mathcal R, \iota(w)=c} \vert \mathcal{P}(w, q) \vert$, where $\mathcal{P}(w, q)$ is the set of paths from $q_0$ to $q$ in $\mathcal{A}$ labelled by $w$.
Note, that for DFAs, we have $|\mathcal{P}(w,q)|=1$.
The words which have at least $k$ arches in their arch factorisation are captured in the auxiliary $n \times m + 1$ size table $U[q, \ell]$, which we refer to as the \emph{universal words table}. Each entry in $U$ is indexed by a state $q \in Q$ and length $\ell \in [0, m]$ with the entry $U[q, \ell]$ containing the number of $\ell$-length paths ending at $q$ which are $k$-universal, i.e., $\iota(w)\geq k$.

%\begin{remark}
%In the case of NFA, we have $q\in\delta(q_0,w)$ both in $T[q,\ell,c,\mathcal{R}]$ and $U[q,\ell]$.
%\end{remark}

The remainder of this section provides the combinatorial and technical tools needed to construct the tables $T$ and $U$.
Theorems \ref{thm:counting_exactly_ell_k_subsequence_universal_words} and \ref{thm:counting_everything}, and Corollary \ref{col:counting_up_to_ell_k_subsequence_univeral_words} summarise the main complexity results of this section.

% \begin{lemma}
%     \label{lem:nessesary_conditions_for_lengthing_the_paths}
%     Given the automaton $\mathcal{A}$, for every $\ell$-length path ending at state $q$ with $c$-arches and the set of symbols $\mathcal{R}$ in the suffix, the $(\ell - 1)$-length prefix of this path ending at the state $q'$, such that $\delta(q', x) = q$, must satisfying one of the following:
%     \begin{itemize}
%         \item if $\mathcal{R} \neq \emptyset$ then the $(\ell - 1)$-length path $P[1, \ell - 1]$ must correspond to some word with $c$-arches and a (possibly empty) suffix with the set of symbol $\mathcal{R}'$ such that $\mathcal{R}' \cup \{x\} = \mathcal{R}$, where $x$ is the symbol such that $\delta(P[\ell - 1], x) = q$,
%         \item if $\mathcal{R} = \emptyset$, then the $(\ell - 1)$-length path $P[1, \ell - 1]$ must correspond to some word with $c - 1$ arches and suffix with the set of symbols $\mathcal{R}'$ such that $\mathcal{R}' \cup \{x\} = \Sigma$.
%     \end{itemize}
%     Further, any path of length $(\ell - 1)$ satisfying these conditions and ending at the state $q'$ 
% \end{lemma}

% \begin{proof}
%     In the first case, in order for the path ending at $q$ to both contain $c$-arches, and non-empty suffix, the path $P[1, \ell - 1]$ must contain $c$-arches.
%     Further, for the suffix to contain the set of symbols $\mathcal{R}$, either the set of symbols $\mathcal{R}'$ in the suffix of $P[1, \ell - 1]$ must equal $s$, and $x \in \mathcal{R}$, or $\mathcal{R}' = \mathcal{R} \setminus \{x\}$, and hence $\mathcal{R} = \mathcal{R}' \cup \{x\}$.

%     In the second case, the suffix of $P$ can be empty if and only if the transition between $P[\ell - 1]$ and $q$ corresponds to the last symbol in the $c^{th}$ arch.
%     Therefore, $P[1, \ell - 1]$ must contain $c - 1$ arches, followed by a suffix containing the set of symbols $\Sigma \setminus \{x\}$.

%     In the other direction, given a path $P$ of length $\ell - 1$ satisfying these conditions and ending at the state $q'$, the path $P'$ formed by concatenating the transition from $q'$ labelled $x$ will be an $\ell$-length path with $c$-arches and containing a suffix with the set of symbols $\mathcal{R}$.
% \end{proof}

% \todofda{Re-start updating the notation here}

\begin{lemma}
    \label{lem:making_a_path_longer}
    Let $\pi$ be an $(\ell - 1)$-length path in the NFA $\mathcal{A}$ ending at $q$ and corresponding to the word $w_{\pi}$, such that $\iota(w_{\pi}) = c$ and $\letters(\r(w_{\pi})) = \mathcal{R}$. % containing $c$ arches and the set of symbols $\mathcal{R}$ in the post arch suffix.
    Then the word $w_{\pi'}$ corresponding to the path $\pi'$ formed by following a transition labelled $\tx\in\Sigma$ from $q$ either:
    \begin{itemize}
        \item has an empty rest $(\r(w_{\pi'}) = \varepsilon)$ if $\mathcal{R} \cup \{\tx\} = \Sigma$ and hence $\iota(w_{\pi'}) = c + 1$, or% and $\r(w_{p'}) = \varepsilon$, or
        \item has a rest equal to $\mathcal{R} \cup \{ \tx \}$ $(\letters(\r(w_{\pi'})) =  \mathcal{R} \cup \{\tx\})$ if $\mathcal{R} \cup \{\tx\} \subsetneq \Sigma$ and hence $\iota(w_{\pi'}) = c$. % and $\letters(\r(w_{p'})) =  \mathcal{R} \cup \{x\}$. %if $\mathcal{R} \cup \{x\} \neq \Sigma$.
    \end{itemize}
\end{lemma}
\ifpaper
\else
\input{proofs/making_a_path_longer.tex}
\fi

Lemma \ref{lem:making_a_path_longer} provides the outline of the dynamic programming approach used to compute the table $T$.
Starting with the $0$-length path corresponding to the empty word $\varepsilon$, the value of $T[q, \ell, c, \mathcal{R}]$ is computed from the values of $T[q', \ell - 1, c', \mathcal{R}']$, allowing an efficient computation of the table.
Corollary \ref{lem:path_prefixes} rewrites this in terms of computing the number of paths of length $\ell$ ending at state $q$ corresponding to words with $c$ arches and the set of symbols $\mathcal{R}$ of $w$'s rest. The proof is analogous to the one of Lemma~\ref{lem:making_a_path_longer}.

\begin{corollary}
    \label{lem:path_prefixes}
    Let $\pi$ be an $\ell$-length path in the NFA $\mathcal{A}$ with $\iota(w_{\pi}) = c$, and $\al(\r(w_{\pi})) = \mathcal{R}$.
    Now, we distinguish the cases whether $\mathcal{R}$ is empty:
    \begin{description}
    \item[$\mathcal{R}=\emptyset$:]  $\iota(w_{\pi}[1, \ell - 1]) = c - 1$ and $\al(\r(w_{\pi}[1, \ell - 1])) = \Sigma \setminus \{ w_{\pi}[\ell] \}$,
    \item[$\mathcal{R}\neq\emptyset$:] $\iota(w_{\pi}[1, \ell - 1]) = c$ and 
    either $\al(\r(w_{\pi}[1, \ell - 1])) = \al(r(w_{\pi})) \setminus \{w_{\pi}[\ell] \}$ or $\al(\r(w_{\pi}[1, \ell - 1])) = \al(\r(w_{\pi}))$. In this case we also have $\mathcal{R} = \al(r(w_{\pi}[1, \ell - 1])) \cup \{w_{\pi}[\ell] \}$.
    \end{description}
%     Then, either \\
%     if $\mathcal{R} = \emptyset$, then $\iota(w_{\pi}[1, \ell - 1]) = c - 1$ and $\al(\r(w_{\pi}[1, \ell - 1])) = \Sigma \setminus \{ w_{\pi}[\ell] \}$,\\
%     or\\
%     if $\mathcal{R} \neq \emptyset$, then $\iota(w_{\pi}[1, \ell - 1]) = c$ and \\
%     either $\al(\r(w_{\pi}[1, \ell - 1])) = \al(r(w_{\pi})) \setminus \{w_{\pi}[\ell] \}$ or $\al(\r(w_{\pi}[1, \ell - 1])) = \al(\r(w_{\pi}))$,\\
%     and hence $\mathcal{R} = \al(r(w_{\pi}[1, \ell - 1])) \cup \{w_{\pi}[\ell] \}$.
\end{corollary}

Now, we formally establish the dynamic programming approach to calculate the value of $T[q,\ell,c,\mathcal{R}]$ from the already computed cells of the table. For better readability, we use $\mathcal{P}[q,\ell,c,\mathcal{R}]$ as the set of all $\ell$-length paths from $q_0$ to $q$ where the associated word has $c$ arches and the alphabet of its rest is $\mathcal{R}$. Notice that we have $|\mathcal{P}[q,\ell,c,\mathcal{R}]|=T[q,\ell,c,\mathcal{R}]$.

\begin{lemma}
    \label{lem:number_of_paths}
    Let $\mathcal{A}$ be an NFA and assume that $T[q_0,0,0,\emptyset]$ is given.
    Notice that given $q\in Q$, the combination $(q',\tx)\in Q\times\Sigma$ only contributes to $T[q,\ell,c,\mathcal{R}]$ if we have $q'\in\Delta(q,\tx)$. Thus, we have for all $\ell\geq 1$    
    $$ 
    T[q, \ell, c, \mathcal{R}] =
        \sum\limits_{\overset{\tx \in \Sigma,}{q'\in\Delta(q,\tx)}} \begin{cases}
            0 & \mbox{if }\tx \notin \mathcal{R} \text{ and } \mathcal{R} \neq \emptyset,\\
            0 & \mbox{if }\mathcal{R} = \emptyset, c = 0,\\
            T[q', \ell - 1, c - 1, \Sigma \setminus \{\tx\}] & \mbox{if } \mathcal{R} = \emptyset, c > 0, \\
                T[q', \ell - 1, c, \mathcal{R} \setminus \{\tx\}] 
                + T[q', \ell - 1, c, \mathcal{R}]
                 & \mbox{if }\mathcal{R} \neq \emptyset, x \in \mathcal{R}.
        \end{cases}
    $$
\end{lemma}
\ifpaper
\else
\input{proofs/number_of_paths.tex}
\fi

Following Lemma \ref{lem:number_of_paths}, the table $T$ can be constructed via dynamic programming. % approach.
As a base case, note that the only length $0$ path in this automaton starting at $q_0$ is the empty path, which must also end at state $q_0$ and contains $0$ arches and no symbols in the alphabet of the rest.
Therefore, $T[q, 0, c, \mathcal{R}]$ is set to $0$ for every $q \in Q, \mathcal{R} \subsetneq \Sigma$ and $c \in [0, k-1]$ other than $T[q_0, 0, 0, \emptyset]$, which is set to 1.
We now use $T$ to construct $U$.
%
% For length $1$ paths, the value of $T[q, 1, c, \mathcal{R}]$ is set to $1$ for every $q \in Q, \mathcal{R} \subseteq \Sigma$ such that $\mathcal{R} = \{\tx\}$ for some $\tx \in \Sigma$ such that $q\in \Delta(q_0, x)$. Recall that we assume to have at least a binary alphabet and thus a single letter does not build an arch.
% The remaining entries are set to $0$.
% In the general case, we use the following technical lemma, rewording Lemma \ref{lem:number_of_paths} in terms of the table $T$.
% The following lemma includes the computation of $U$ as an extension of $T$ and the runtime of the computation.


\begin{corollary}
    \label{col:generally_computing_the_path_table}
    We have
    $U[q,\ell]= \sum_{\tx \in \Sigma,q'\in\Delta(q,\tx)} 
    		U[q', \ell - 1] + T[q', \ell - 1, k - 1, \Sigma \setminus \{\tx\}]$.
    % Further, the values of $T[q, \ell, c, \mathcal{R}]$ and $U[q, \ell]$ can be computed for every $q \in Q, \ell \in [0, m], c \in [0, k - 1]$ and $\mathcal{R} \subsetneq \Sigma$ in $O(m n^2 k \sigma 2^{\sigma})$ time.
\end{corollary}
\ifpaper
\else
\input{proofs/generally_computing_the_path_table.tex}
\fi

% Note that Lemma \ref{lem:generally_computing_the_path_table} is consistent with the above explanation of length 1 paths.
Note that the total number of $k$-universal accepting paths of the automaton $\mathcal{A}$ is given by $\sum_{q \in F} U[q, m]$.
Using the tables $T$ and $U$, the total number of $k$-universal paths and words of length $m$ can be computed in 
% $O(m^2 n^2 k \sigma 2^{\sigma})$.
$O^*(m^2 n^2 k 2^{\sigma})$.

\begin{theorem}
    \label{thm:counting_exactly_ell_k_subsequence_universal_words}
    The number of $k$-universal accepting paths of length $m$ of  an NFA $\mathcal{A}$, for $k\leq m/\sigma$, can be computed in 
    $O^*(m^2 n^2 k 2^{\sigma})$
    % $O(m^2 n^2 k \sigma 2^{\sigma})$
    time. For  $k> m/\sigma$, this number is $0$.
\end{theorem}
\ifpaper
\else
\input{proofs/counting_exactly_ell_k_subsequence_universal_words.tex}
\fi

\begin{corollary}
    \label{col:counting_up_to_ell_k_subsequence_univeral_paths}
    The number of  $k$-universal accepting paths of length at most $m$ of an NFA $\mathcal{A}$, for $k\leq m/\sigma$, can be computed in 
    % $O(m^2 n^2 k \sigma 2^{\sigma})$
    $O^*(m^2 n^2 k 2^{\sigma})$
    time. For  $k> m/\sigma$, this number is $0$.
\end{corollary}

\ifpaper
\else
\input{proofs/col_counting_up_to_ell_k_subsequence_univeral_paths.tex}
\fi

Since in a DFA each word is associated with exactly one path, the following holds.

\begin{corollary}
    \label{col:counting_up_to_ell_k_subsequence_univeral_words}
    The number of $k$-universal words of length either exactly or at most $m$ accepted by a DFA $\mathcal{A}$, for $k\leq m/\sigma$, can be computed in 
    % $O(m^2 n^2 k \sigma 2^{\sigma})$ 
    $O^*(m^2 n^2 k 2^{\sigma})$ 
    time. For  $k> m/\sigma$, this number is $0$.
\end{corollary}

% \begin{corollary}
%    \label{col:counting_up_to_ell_k_subsequence_univeral_words}
%    The number of  $k$-universal words of length at most $m$ accepted by the automaton $\mathcal{A}$ can be computed in $O(m n^2 k \sigma 2^{\sigma})$ time.
% \end{corollary}

% \ifpaper
% See Example~\ref{example} in the appendix for an example of these algorithms.
% \else
% \begin{example}\label{example}
% Consider again the automaton $\mathcal{A}$ from Figure~\ref{img:universal_automaton}. Let $k=2$. We have $T[q_0,0,0,\emptyset]=1$ and $T[q_0,1,0,\{\ta\}]=T[q_0,1,0,\{\tb\}]=T[q_1,1,0,\{\tc\}]=1$.
% For the path of length $2$, we have the words $\ta\ta,\ta\tc,\tb\ta,\tb\tc$, and $\tc\ta$. Thus, we have
% \begin{align*}
% T[q_0,2,0,\{\ta\}] &=T[q_0,1,0,\emptyset]+T[q_0,1,0,\{a\}]=0+1=1,\\
% T[q_0,2,0,\{\ta,\tb\}] &= T[q_0,1,0,\{\tb\}]+T[q_0,1,0,\{\ta,\tb\}]=1+0=1,\\
% T[q_1,2,0,\{\tx,\tc\}] &= T[q_0,1,0,\{\tx\}]+T[q_0,1,0,\{\tx,\tc\}]=1+0=1,\forall \tx\in\{\ta,\tb\},\\
% T[q_2,2,0,\{\tc,\ta\}] &= T[q_1,1,0,\{\tc\}]+T[q_1,1,0,\{\tc\}]=1+0=1.
% \end{align*}
% For words of length $3$ and $4$, we get the following values (all others are $0$).
% \begin{center}
% \begin{tabular}{cccc|c}
% $q'$ & $\ell$ & $c$ & $\mathcal{R}$ & amount \\ \hline
% $q_0$ & 3& 0 &$\{\ta\}$ & $1$ \\
% $q_0$ & 3& 0 &$\{\tb\}$ & $1$ \\
% $q_0$ & 3& 0 &$\{\ta,\tb\}$ & $6$ \\
% $q_1$ & 3& 0 &$\{\ta,\tc\}$ & $1$ \\
% $q_1$ & 3& 0 &$\{\tb,\tc\}$ & $1$ \\
% $q_1$ & 3& 1 &$\emptyset$ & $2$ \\
% $q_2$ & 3& 1 &$\emptyset$ & $2$ \\
% $q_2$ & 3& 0 &$\{\ta,\tc\}$ & $1$ 
% \end{tabular}
% \hspace{1cm}
% \begin{tabular}{cccc|c}
% $q'$ & $\ell$ & $c$ & $\mathcal{R}$ & amount \\ \hline
% $q_0$ & 4& 0 &$\{\ta\}$ & $1$ \\
% $q_0$ & 4& 0 &$\{\tb\}$ & $1$ \\
% $q_0$ & 4& 0 &$\{\ta,\tb\}$ & $14$ \\
% $q_1$ & 4& 0 &$\{\ta,\tc\}$ & $1$ \\
% $q_1$ & 4& 0 &$\{\tb,\tc\}$ & $1$ \\
% $q_1$ & 4& 1 &$\emptyset$ & $6$ \\
% $q_2$ & 4& 0 &$\{\ta,\tc\}$ & $3$ \\
% $q_2$ & 4& 1 &$\{\ta\}$ & $2$ \\
% $q_2$ & 4& 1 &$\{\tb\}$ & $2$ \\
% $q_2$ & 4& 1 &$\{\tc\}$ & $2$ \\
% $q_2$ & 4& 1 &$\emptyset$ & $3$
% \end{tabular}
% \end{center}
% \end{example}
% \fi
We may further generalise this to the problem of finding the number of perfect $k$-universal words and paths by discarding any $k$-universal paths with a non-empty rest.

\begin{corollary}
	\label{col:counting_perfect_universal_paths}
	The number of perfect $k$-universal accepting paths of length either exactly or at most $m$ of an NFA $\mathcal{A}$, for $k\leq m/\sigma$, can be computed in 
	% $O(m^2 n^2 k \sigma 2^{\sigma})$
	$O^*(m^2 n^2 k 2^{\sigma})$
	time.
\end{corollary}


\begin{corollary}
	\label{col:counting_perfect_universal_words}
	The number of perfect $k$-universal words of length either exactly or at most $m$  accepted by a DFA $\mathcal{A}$, for $k\leq m/\sigma$, can be computed in 
	% $O(m^2 n^2 k \sigma 2^{\sigma})$
	$O^*(m^2 n^2 k 2^{\sigma})$
	time.
\end{corollary}

% \begin{corollary}
%	\label{col:counting_perfect_universal_paths}
%	The number of perfect $k$-universal accepting paths of length at most $m$ of a NFA $\mathcal{A}$ can be comptued in $O(m n^2 k \sigma 2^{\sigma})$ time.
%\end{corollary}
%\ifpaper
%\else
%\input{proofs/counting_perfect_universal_paths.tex}
%\fi
%
%\begin{corollary}
%	\label{col:counting_perfect_universal_words}
%	The number of perfect $k$-universal words of length at most $m$  accepted by a deterministic finite automaton $\mathcal{A}$ can be comptued in $O(m n^2 k \sigma 2^{\sigma})$ time.
%\end{corollary}

We now generalise these tools to the problem of counting the total number of $k$-universal paths accepted by a finite automaton $\mathcal{A}$.
The primary challenge of counting the total number of such paths comes from determining if there exists either a finite or an infinite number of $k$-universal paths accepted by $\mathcal{A}$.
%
%We first provide a set of combinatorial lemmas placing an upper bound on the length of the shortest $k$-universal path.
%We phrase these in terms of words for notational simplicity, noting that these results can be directly generalised to $k$-universal paths.
%
%% \begin{lemma}
%%    \label{lem:maximum_path_length}
%%    Given two state $q, q' \in Q$ in the automaton $\mathcal{A}$, there exists a path from $q$ and $q'$ if and only if there exists a path of length at most $n - 1$ from $q$ to $q'$.
%% \end{lemma}
%%
%%\begin{proof}
%%    As there are at most $n$ states in $Q$, the longest path in $\mathcal{A}$ that does not contain a cycle must have a length of at most $n - 1$.
%%    Hence if there exists a path from $q$ to $q'$, there must exist some path from $q$ to $q'$ of length at most $n - 1$.
%%\end{proof}
%
%\begin{lemma}
%    \label{lem:reaching_every_state_further}
%    Given a pair of states $q, q' \in Q$ in the automaton $\mathcal{A}$ such that there exists a path $P$ from $q$ to $q'$ where the final transition in $P$ is labelled $\tx \in \Sigma$.
%    Then, there exists some path $P'$ of length at most $n$ from $q$ to $q'$ where the final transition in the path is labelled $\tx$.
%    % there either exists some path from $q$ to $q'$ of length at most $n$ containing the symbol $\tx$, or there exists no paths from $q$ to $q'$ containing the symbol $\tx$.
%\end{lemma}
%\ifpaper
%\else
%\input{proofs/reaching_every_state_further.tex}
%\fi
%
%\begin{lemma}
%	\label{lem:ksu_min_length}
%	Given an automaton $\mathcal{A}$ with $n$ states, if there is a $k$-universal word accepted by $\mathcal A$, then there is a $k$-universal word accepted by $\mathcal{A}$ of length at most $k n \sigma$.
%\end{lemma}
%\ifpaper
%\else
%\input{proofs/ksu_min_length.tex}
%\fi
%
%An example of an automaton for which the shortest $k$-universal word has length $k (n \sigma - 1)-(k-1)(n-1)$\todo{change Figure 3 accordingly} is given in Figure~\ref{img:worstcaseexample}.
%
%
By the pumping lemma \cite{HopcroftU79}, we have that an automaton $\mathcal{A}$ accepts an infinite number of $k$-universal words (paths) if and only if $\mathcal{A}$ accepts some $k$-universal word (path) of length at least $n + 1$. Clearly, if $k>n$ we have that $\mathcal{A}$ either accepts an infinite number of $k$-universal words (paths) or none (and this can be tested as in Lemma \ref{lem:ESUPFA}, in time that does not depend on $k$). Therefore, using the upper bound on the maximum length of the shortest $k$-universal word accepted by the automaton $\mathcal{A}$ from Lemma \ref{lem:ksu_min_length}, 
% we now have an upper bound on the maximum length of the shortest $k$-universal word accepted by the automaton $\mathcal{A}$.
combined with Corollary \ref{col:counting_up_to_ell_k_subsequence_univeral_words}, we now count the total number of $k$-subsequence universal words accepted by $\mathcal{A}$.\looseness=-1

\begin{theorem}
\label{thm:counting_everything}
    The total number of $k$-universal words (resp., paths) accepted by a DFA (resp., NFA) $\mathcal{A}$ can be determined in 
    $O^*(n^4 k^2 2^{\sigma})$ time (resp.,  $O^*(n^4 k^3 2^{\sigma})$ time),
    % $O(n^4 k^2 \sigma^2 2^{\sigma})$ time (resp.,  $O(n^4 k^3 \sigma^3 2^{\sigma})$ time),
   for $k\leq n$. For $k> n$, this number is either $0$ or $\infty$, and can be determined in
     $O^*(n^3 2^\sigma)$ time. 
     % $O(n^3 \sigma^2 2^\sigma)$ time. 
\end{theorem}
\ifpaper
% \input{proofs/counting_everything.tex}
\else
\input{proofs/counting_everything.tex}
\fi



% \todo{unsure how to embbedd this nicely in the proof, another remark or just as a text is between}
% The worst case scenario described in Theorem~\ref{thm:counting_everything} is visible in Figure~\ref{img:worstcaseexample}.

% The next result follows in the same way.

%\begin{corollary}
%	\label{col:counting_every_path}
%	The total number of $k$-universal paths accepted by an NFA $\mathcal{A}$ can be determined in $O(n^4 k^3 \sigma^3 2^{\sigma})$ time.
%\end{corollary}


%\subsection{Solving \texorpdfstring{$k$}{k}-ASUPFA and \texorpdfstring{$k$}{k}-ESUPFA}
%
%We now show that our tools for counting the number of $k$-universal words accepted by an automaton $\mathcal{A}$ can be applied to solve $k$-ASUPFA and $k$-ESUPFA.
%
%\begin{theorem}
%    \label{thm:solving_existance}
%    $k$-ASUPFA can be solved for an $n$ state automaton $\mathcal{A}$ in $O(n^4 k \sigma 2^{\sigma})$ time.
%\end{theorem}
%\ifpaper
%\else
%\input{proofs/solving_existance.tex}
%\fi
%
%% In order to solve $k$-ESUPFA, it is first necessary to provide an upper bound on the length of the shortest $k$-universal word.
%
%
%\begin{theorem}
%    \label{thm:ESUPFA_solving}
%    $k$-ESUPFA can be solved for an automaton $\mathcal{A}$ with $n$ states and an alphabet of size $\sigma$ in $O(n^3 k^2 \sigma^2 2^{\sigma})$ time.
%\end{theorem}
%\ifpaper
%\else
%\input{proofs/ESUPFA_solving.tex}
%\fi
%
%% We note that both our solutions to $k$-ASUPFA and $k$-ESUPFA can be seen as fixed-parameter tractable algorithms relative to the size of the alphabet.
%
%\begin{theorem}
%    \label{thm:polynomail_time_for_constant_alphabets}
%    $k$-ASUPFA and $k$-ESUPFA problems are in FPT when parameterised by the size of the alphabet. 
%    %  can be solved in $O(n^3 k^2)$ time for automata defined over a constant size alphabet.
%\end{theorem}

We now extend our results of counting to the problem of ranking $k$-universal words.
Note, that these results can be generalised to ranking the $k$-universal accepted paths, but one needs to define an ordering on the transitions from each state in the automaton. To keep the presentation simple, we will therefore only discuss here about DFAs and words.
The main idea is to count the number of $k$-universal words with a prefix strictly smaller than the prefix of $w$ of the same length; again, each arithmetic operation takes $O(m)$ time in our computational model.
This section is laid out as follows.
First, we show how to compute the rank of $w$ efficiently within the set $\Univ_{\mathcal{A}_{\leq m}, k}$ in 
$O^*(m^2 n^2 k 2^{\sigma})$ time.
% $O(m^2 n^2 k \sigma 2^{\sigma})$ time.
% We build on this by showing that the rank of $w$ within $\Univ_{\mathcal{A}_{\leq n}, k} $ with the same complexity as finding the $n$-length rank of $w$, improving on the direct approach of simply finding the $i$-length rank of $w$ for every $i \in [1, n]$.
Secondly, we show that the rank of $w$ can be computed within the set $\Univ_{L(\mathcal{A}), k}$ in 
$O^*(n^4 k^3 2^{\sigma})$ time.
% $O(n^4 k^3 \sigma^3 2^{\sigma})$ time.
As noted above, when discussing counting, these problems only make sense for $k\leq m/\sigma$. 
%  the set of all $k$-universal words accepted by $\mathcal{A}$.
This follows from the same arguments used to count the total number of $k$-universal words accepted by $\mathcal{A}$ laid out in Theorem \ref{thm:counting_everything}. \looseness=-1

% We define three related variations of the ranking problem.

% \begin{definition}
%    The \emph{$n$-length rank} of a word $w$ within the set $\Univ_{\mathcal{A}^n, k} $ % $\mathcal{U}(\mathcal{A})$
%    is the number of words in  $\Univ_{\mathcal{A}^n, k}$ that are lexicographically smaller than $w$.
%\end{definition}

%\begin{definition}
%    The \emph{at-most-$n$-length rank} of a word $w$  within the set $\Univ_{\mathcal{A}^n, k}$ is the number of words in 
%    $\Univ_{\mathcal{A}^{ \leq n}, k}$
    % $\mathcal{U}(\mathcal{A}) \cap \left( \bigcup_{i \in [1, n]} \Sigma^{i} \right)$
%     that are lexicographically smaller than $w$.
%\end{definition}

%\begin{definition}
    %The \emph{any-length rank} of a word $w$ within the set $\Univ_{\mathcal{A}, k}$ %$\mathcal{U}(\mathcal{A})$
    %is the number of words in $\Univ_{\mathcal{A}, k}$ % $\mathcal{U}(\mathcal{A})$
    %that are lexicographically smaller than $w$.
%\end{definition}


The primary tool used in this section is a generalisation of the path table: the \emph{fixed prefix path table of length $m$} is an $n \times (m + 1)\times k \times 2^{\sigma}$ sized table, defined for a set of prefixes $\mathcal{PR}$ and denoted $T(\mathcal{PR})$.
Informally, the table $T(\mathcal{PR})$ is used to count the number of paths with some prefix from the given set 
$\mathcal{PR}$. Thus, $T(\mathcal{PR})[q, \ell, c, \mathcal{R}]$ stores the number of words $w\in\Sigma^{\ell}$
associated to a path from $q_0$ to $q$, with $\iota(w)=c$, $\letters(r(w))=\mathcal{R}$, and there exists a $p\in\mathcal{PR}$ such that $p=w[1,|p|]$.
The table $U(\mathcal{PR})$ is defined analogously to the table $U$ but again with the additional condition as in $T(\mathcal{PR})$.
These tables can be constructed directly using the same techniques introduced for $T$ and $U$, by initially setting $T(\mathcal{PR})[q_0, 0, 0, \emptyset]$ to 0 and $T(\mathcal{PR})[\delta(q_0, p), \lvert p \rvert, \iota(p), \letters(\r(p))]$ to $1$ for every $p \in \mathcal{PR}$. % where $q_p$ is the state reached by following the path from $q_0$ labelled by $p$.
Similarly, in the special case where there exists some $p \in \mathcal{PR}$ such that $\iota(p) \geq k$, then the value of $U[\delta(q_0, p), \lvert p \rvert ]$ is set to 1.
We assume, without loss of generality, that no prefix in $\mathcal{PR}$ is also the prefix of some other word $p' \in \mathcal{PR}$.
The remaining entries are computed as before.
In the following results, we use $\mathcal{PR}(w) = \{w[1, i] \tx \mid i \in [0, \lvert w \rvert ], \tx \in [1, w[i + 1] - 1] \}$.
Note, that the following results hold for both counting words accepted by deterministic automata, and accepting paths in non-deterministic automata.

\begin{corollary}
    \label{col:constructing_the_fixed_perfix_table}
    $T(\mathcal{PR})$, $U(\mathcal{PR})$ are constructible for $m$-length paths in % $O(m^2 n^2 k \sigma 2^{\sigma})$ time.
    $O^*(m^2 n^2 k 2^{\sigma})$ time.
\end{corollary}

% Theorem \ref{thm:ranking_fixed_length} follows.

\begin{theorem}
    \label{thm:ranking_fixed_length}
    The rank of $w \in \Univ_{\mathcal{A}_m, k}$ can be determined
    % in $O(m^2 n^2 k \sigma 2^{\sigma})$ time.
    in $O^*(m^2 n^2 k 2^{\sigma})$ time.
\end{theorem}
\ifpaper
%\input{proofs/ranking_fixed_length.tex}
\else
\input{proofs/ranking_fixed_length.tex}
\fi

\begin{corollary}
    \label{col:ranking_up_to_k_length}
    The rank of $w\in \Univ_{\mathcal{A}_{\leq m}, k}$ can be determined 
    % $\mathcal{U}(\mathcal{A})$
    in $O^*(m^2 n^2 k  2^{\sigma})$ time.
    % in $O(m^2 n^2 k \sigma 2^{\sigma})$ time.
\end{corollary}
\ifpaper
\else
\input{proofs/ranking_up_to_k_length.tex}
\fi

\begin{corollary}
    \label{col:ranking_everything}
    The rank of $w \in \Univ_{L(\mathcal{A}), k}$ can be determined in $O^*(n^4 k^3 2^{\sigma})$ time.
    % $O(n^4 k^3 \sigma^3 2^{\sigma})$ time.
\end{corollary}
\ifpaper
\else
\input{proofs/ranking_everything.tex}
\fi



==> proofs/proof_FPT_states_acyclic.tex <==
\begin{proof}
	This follows from the proof of Theorem \ref{thm:FPT_states}. Note that, in this case, each strongly connected component of a state contains a single state, and $V_q=\emptyset$ for all $q\in Q$. So, sorting topologically the strongly connected components corresponds to sorting topologically the states of $A$. In general, the whole process can be implemented more efficiently.
	
	We iterate over all subsets $Q'=\{q_0,f\}\cup \{q_1,\ldots,q_{h-1}\}$ of $Q$; for simplicity, set $q_h=f$ and note that $h< n$.We sort $Q'$ w.r.t. the topological sorting of the states of $A$ (which can be done in $O(n)$ time, as we already have the topological sorting of $S(A)$). After this step, and a potential relabelling of the states, we can assume that $q_{i-1}$ comes before $q_{i}$ for all $i\in [h]$ (and $q_h=f$ still holds). Then, we simply use Lemma \ref{lem:algo_one_seq} for the sequence $q_0\cdots q_h$ of $h< n$ states, as the conditions from the statement of this lemma are fulfilled. The complexity of the algorithm implements in this lemma is now only $O(n^3\sigma^{1.5})$. We then store the maximum value $k$ computed in the respective lemma (over all the considered sequences $q_0\cdots q_h$). This is the maximum universality of a word of $L$. As the number of the considered subsets is $O(2^n)$, the statement follows.
\qed \end{proof}

==> proofs/proof_commutative_finite_k.tex <==
\begin{proof}
	Let $\mathcal A = (Q,\Sigma, \delta, q_0, F)$ with $|Q| = n$ and $L(\mathcal A) = L$.  Now, let $q$ be the state reached by following the path $\pi_{w}$ for $w = \ta^k \tb^k \cdots \sigma^k$. Note that, as $\mathcal{A}$ is commutative, if there exists any word containing $k$ arches, there must also exist some word with the prefix $w$. Therefore, if $q$ is either an accepting state, or can reach an accepting state by some set of transitions, there exists some set of $k$-subsequence universal words in $L$. Otherwise, no such word exists. As we can determine if any such path exists in $O(n \sigma)$ time via a depth-first search, we obtain the complexity.\qed
	%
	% Check whether the path $a^k b^k \cdots \sigma^k$ ends in an accepting state or a state that can reach an accepting state by following.
	% one transition apart from an accepting state. Since the automaton is a DFA, there is a unique path for $a^k b^k \cdots \sigma^k$. Thus, we can verify this in $O(\sigma k)$.
\end{proof}

==> proofs/proof_commutative_infinite_k.tex <==
\todo[inline]{this is not better than the respective lemma for regular languages, we could just as well test $(ab\ldots\sigma)^{n+1}$.\\ Edit: It is better in the sense that we can also use this approach for $k\leq n$. If there is a k-universal word in L we can also find a word with prefix $a^kb^k\ldots\sigma^k$. Still, can we decide whether such a wort exists in L? Should be possible by removing non-(co-)accessible states and then check whether we are still alive after reading $a^kb^k\ldots\sigma^k$.}

\begin{proof}
	Consider the word $w = \ta^{n + 1} \tb^{n + 1} \dots \sigma^{n + 1}$. Observe that if there exists some $v\in \Sigma^*$ such that $w v \in L$, then the path induced by $w$ must include at least one cycle labelled by each symbol in $\Sigma$. Let $\ell_{i}$ be the length of the cycle in $\mathcal A$ taken by the walk induced by $w$ labelled by the symbol $i \in \Sigma$. Then, as  $w v \in L$, we have that $ \ta^{n + 1 + c \cdot \ell_\ta} \tb^{n + 1 + c \cdot \ell_\tb} \cdots \sigma^{n + 1 + c \cdot \ell_{\sigma}} v \in L$, for all $c \in \mathbb{N}$.
	In the other direction, of $L$ is not $(n + 1)$-ESU, then $L$ can not be $k$-ESU for any $k \geq n + 1$.
	Therefore, we can determine the statement in $O(n \sigma)$ time by checking if $L$ is $(n + 1)$-ESU, requiring, by Proposition \ref{prop:commutative_finite_k}, $O(n \sigma)$ time.\qed
\end{proof}

==> proofs/proof_construction_L_table.tex <==
\begin{proof}
	We prove this in an inductive manner. Observe that $L[0, s]$ is $False$ for every $s \subseteq \Sigma, s \neq \emptyset$, and $True$ for $L[0, \emptyset]$. Now, let us assume that for every $\ell' \in [1, \ell - 1]$, and $s \subset \Sigma$, $L[0, s]$ has been properly computed. Then $L[\ell, s]$ will be true if and only if there exists some state $q$ such that $\delta(q, x) = q_{\ell}$, for some $x \in \Sigma$, and $L[\ell, s \setminus \{ x \}]$, meaning that there exists some word $u \in \Sigma^+$ such that $\delta(q_0, u) = q$ and $s \setminus \{ x \} \subseteq \letters(u)$, and thus $s \subseteq \letters(u x)$. Therefore, if $L[q, s \setminus \{ x \}]$ is true for some $(q, x) \in P_{\ell}$, $L[\ell, s]$ is also true. In the other direction, if $L[q, s \setminus \{ x \}]$ is false for every $(q, x) \in P_{\ell}$, then there is no path ending at $q_{\ell}$ corresponding to a word $u \in \Sigma^+$ such that $s \subseteq \letters(u)$, and hence $L[\ell, s]$ is false.\qed
\end{proof}

==> proofs/proof_construction_U_table.tex <==
\begin{proof}
	We prove this in an inductive manner. Note that $U[0, s] = 0$, for every $s \subset \Sigma$. Now, assume that $U[q_{\ell'}, s]$ is properly computed for every $\ell' \in [1, \ell - 1]$ and $s \subset \Sigma$.
	
	First, we consider the case where $s \neq \emptyset$. 
	Note that given any word $u \in \Sigma^+$ such that $\delta(q_0, u) = q$, and $x \in \r(u)$, for any pair $q, x \in P_{\ell}$, we have, by definition, $U[\ell, s] \geq \iota(u)$, and thus $U[\ell, s] \geq U[q, s]$. Equivalently, we have that, for any $u \in \Sigma^+$ where $\delta(q_0, u) = q$ and $s \setminus x \subseteq \r(u)$, $U[\ell, s] \geq \iota(u)$, and thus $U[\ell, s] \geq U[q, s \setminus \{ x \}]$. Further, as $s \setminus \{ x \} \subseteq s$, we have, by construction, that $U[q, s \setminus \{ x \}] \geq U[q, s]$. Therefore, we have that $U[\ell, s] \geq max_{(q, x) \in P_{\ell, s}} U[q, s \setminus x]$ when $s \neq \emptyset$. To show that $U[\ell, s] = \max_{(q, x) \in P_{\ell, s}} U[q, s \setminus x]$, observe that $U[\ell, s] > \max_{(q, x) \in P_{\ell, s}} U[q, s \setminus \{ x \}]$ only if there exists some word $u$ containing at least $\vert s \vert + 1$ new symbols, representing a new arch and the number of symbols required to have the set $s$ in the rest of the word, leading to a contradiction as the existence of any such word would imply some $u'$ such that $\delta(q_0, u') = q$ and $\delta(u' x) = q_{\ell}$, thus $U[q, s \setminus \{ x \}] = U[\ell, s]$. Hence, $U[\ell, s] = max_{(q, x) \in P_{\ell, s}} U[q, s \setminus x]$
	
	If $s = \emptyset$, $\ell > 0$, and $L[q_{\ell}, \Sigma]$ is $True$, the value of $U[\ell, s]$ is equal to the greatest universality of any word $u \in \Sigma^*$ such that $\delta(q_0, u) = q_{\ell}$. Therefore we have two possibilities. First, $U[\ell, s]$ may be equal the maximum universality of any word ending at some state $q$ for which $\delta(q, x) = q_{\ell}$ for some $x \in \Sigma$, equal to $\max_{q, x \in Q_{\ell, \sigma}} U[\ell, \emptyset]$. Otherwise, $U[\ell, s]$ is formed by extending some word $u \in \Sigma^+$ such that $\delta(q_0, u) = q$, and $u$ contains a rest $\r(u) = \Sigma \setminus \{ x \}$, where $q, x \in Q_{\ell, \Sigma}$. In this case,  $U[\ell, s] = \max_{(q, x) \in Q_{\ell, 
			\Sigma}} U[\ell, \sigma \setminus \{x \}] + 1$. Hence, $U[\ell, \emptyset] = max\left(\max_{(q, x) \in Q_{\ell, \Sigma}} \left(U[\ell, s \setminus x] + 1 \right),  \max_{(q, x) \in P_{\ell}} U[\ell, \emptyset]\right)$.\qed
\end{proof}

==> proofs/proof_finite_language_is_acyclic.tex <==
\begin{proof}
	We assume, without loss of generality, that there exists, for every state in $\mathcal{A}$, some path ending at an accepting state. Assume now, for the sake of contradiction, that there exists some cycle in $\mathcal{A}$, labelled by the word $w \in \Sigma^*$ starting and ending at the state $q$. Now, let $p \in \Sigma^*$ be some word such that $\delta(q_0, p) = q$, and let $s \in \Sigma^*$ be some word such that $\delta(q, s) = f$, where $q_0$ is the starting state, and $f$ is some accepting state. Then, $\mathcal{A}$ accepts the word $p w^k s$, for any $k \in \mathbb{N}$. \qed
\end{proof}

==> proofs/proof_k-ESU_RLNP.tex <==
\begin{proof}
	Follows from $\NIL \subseteq PL_1^P$.\qed
\end{proof}

==> proofs/proof_k-ESU_acyclic.tex <==
\begin{proof}
	Note that the construction given in  \cite{regunivpaper} to show hardness of general automata uses acyclic automata.\qed
\end{proof}

==> proofs/proof_making_expressions_star_free.tex <==
\begin{proof}
	As there does not exist any Kleene-star terms containing the full alphabet $\Sigma$, we have, by Lemma \ref{lem:unbounded_universality_regex}, that there exists some $k'$ for which $R$ is not $k'$-ESU. We now prove this statement in an inductive manner. Note that this holds by definition for any word matched by the prefix $u_0$. Now, let us assume that for any word $w$ matched by $u_0 s_1 u_1 s_2 \dots u_{\ell - 1}$, this holds. Consider the word $w$ matched by $u_0 s_1 u_1 s_2 \dots u_{\ell - 1} s_{\ell}$ such that, for all $v \in \Sigma^{*}$, either $v$ is not matched by $u_0 s_1 u_1 s_2 \dots u_{\ell - 1} s_{\ell}$, or $\iota(v) \leq \iota(w)$. Further, let $w'$ be the prefix of $w$ matched by $u_0 s_1 u_1 s_2 \dots u_{\ell - 1}$. We consider two cases. If $\iota(w) = \iota(w')$, then note that $\r(w) \subseteq \r(w') \cup \letters(s_{\ell}) = \r(w') \cup \{a_1, a_2, \dots, a_{\alpha_{\ell}}\}$. Therefore, any word $v = w v'$ matched by $R$ satisfies $\iota(w'  a_1 a_2 \dots a_{\alpha_{\ell}} a_1 a_2 \dots a_{\alpha_{\ell}} v') \geq v$. Otherwise, $\iota(w) = \iota(w') + 1$. In this case, note that as $\letters(s_{\ell}) = \{ a_1, a_2, \dots. a_{\alpha_i}\}$, $\r(w) \subseteq \{ a_1, a_2, \dots, a_{\alpha_i}\}$, and hence any word $v = w v'$ matched by $R$ satisfies $\iota(w'  a_1 a_2 \dots a_{\alpha_{\ell}} a_1 a_2 \dots a_{\alpha_{\ell}} v') \geq v$. 
	Note that, as $u_{\ell}$ is star free, if the statement holds for $u_0 s_1 u_1 s_2 \dots u_{\ell - 1} s_{\ell}$, it must also hold for $u_0 s_1 u_1 s_2 \dots u_{\ell - 1} s_{\ell} u_{\ell}$, and therefore the Lemma holds.\qed
\end{proof}

==> proofs/proof_maximal_k_commutative_language.tex <==
\begin{proof}
	We do this by way of a binary search on the values of $k$. Starting with $k = n + 1$, we determine if the value of $k$ is finite via Proposition \ref{prop:commutative_infinite_k} in $O(n \sigma)$ time.
	If $k$ is finite, then we may perform a binary search over the possible values of $k$, starting with $k = n / 2$, and proceeding accordingly. As each $k$ requires $O(n \sigma)$ time to process, and we require at most $\log n$ such checks, the total time complexity of this process is $O(n \sigma \log n)$.\qed
	%	Let $\mathcal A = (Q,\Sigma, \delta, q_0, F)$ with $|Q| = n$ and $L(\mathcal A) = L$. By definition, we know that for an arbitrary $k\in \N$ the strictly $k$-universal word $w$
	%%	with $y \in \Sigma^*$ with $\al(y) \subset \Sigma$ 
	%	is contained in the language iff its sorted permutation $\ta^{\ell_\ta} \tb^{\ell_\tb} \cdots \sigma^{\ell_\sigma}$ is contained for $\ell_i \in \N_{\geq k}$, $i \in [\sigma]$. Thus, we need to find the largest possible powers $\ell_i$ such that $\ta^{\ell_\ta} \tb^{\ell_\tb} \cdots \sigma^{\ell_\sigma}$ is accepted by the automaton. Then the smallest amongst the $\ell_i$ is the largest universality we can reach (the permutation we construct does contain this letter that occurs the fewest as the modus). In order to find the largest possible values for $\ell_i$ we go from the initial state and use the Floyd-Warshall algorithm to compute all pairs of shortest paths between the initial and final states that are of the form $\ta^{\ell_\ta} \tb^{\ell_\tb} \cdots \sigma^{\ell_\sigma}$ (all other pairs are omitted) in $O(n^3)$ time while storing the number of letters $\ell_i$ along the path and possible single letter loops within a block of $\ta^{\ell_\ta} \tb^{\ell_\tb} \cdots \sigma^{\ell_\sigma}$. If every block $\mathtt{i}^{\ell_i}$, $\mathtt{i} \in \Sigma$ contains a loop, there exist $k$-universal words  for every $k\in \N$. If there exists a letter $\mathtt{i} \in \Sigma$ without a loop in its block then we compute the maximal power for each of those letters by counting the number of transitions from the beginning to the end of their block. Let $\ell_j$ for $j \in [\sigma]$ be the smallest value amongst all exponents. Thus, we can conclude that the universality of the language is bounded by $\ell_j$ since $k$ was chosen arbitrarily.
\end{proof}

==> proofs/proof_regex_fixed_universality.tex <==
\begin{proof}
	From Lemma \ref{lem:unbounded_universality_regex} we can determine if this holds by checking if there exists any subexpression of the form $r$ of the form $(r[2, \vert r \vert - 2])^*$ where $\letters(r) = \Sigma$. Note that we can determine if this holds for any given expression $r$ in $O(\vert r \vert)$ time. Further, it is sufficient only to check any subexpressions that are not contained within another Kleene-star, and by extension within another subexpression of the same form. As we can determine the set $r_1, r_2, \dots, r_m$ of candidate expressions in $O(n)$ time by a simple scan of the expression, and $\vert r_1 \vert + \vert r_2 \vert + \dots + \vert r_m \vert \leq n$, we get the statement.\qed
\end{proof}

==> proofs/proof_regex_k_esu.tex <==
\begin{proof}
	From Theorem \ref{thm:regex_fixed_universality} we can determine if $R$ is $k$-ESU for every $k \in \mathbb{N}$ in $O(n)$ time. If this does not hold,  from Lemma \ref{lem:making_expressions_star_free} we may construct a new star-free regular expression $R'$ containing at most $O(n)$ symbols in $O(n)$ time. This can be then converted into an acyclic automaton $\mathcal{A}(R')$ containing $O(n)$ states and $O(\sigma n)$ transitions. By Theorem \ref{thm:universality_of_regex}, we can determine if $\mathcal{A}(R')$, and by extension $R$, is $k$-ESU in $O(\sigma n 2^{\sigma})$ time.\qed
\end{proof}

==> proofs/proof_unbounded_universality_regex.tex <==
\begin{proof}
	In one direction, observe that if some such subexpression exists, then one can create a word $u$ such that $\letters(u) = \Sigma$ matching the subexpression. Therefore, for any given $k$, one may construct a $k$-universal word by including the factor $u^k$. In the other direction, if no such subexpression exists, then there exists some $k'$ such that, for any word $u \in \Sigma^*$ where $u$ is matched by some subexpression of $R$, $\iota(u^m) \leq k'$, for every $m \in \mathbb{N}$. Therefore, $R$ does not satisfy $k''$-ESU of any $k'' \geq k'$, and hence the statement holds.\qed
\end{proof}

==> proofs/proof_universality_of_rexexp.tex <==
\begin{proof}
	From Lemmas \ref{lem:making_table_L} and \ref{lem:making_table_u} we have that the tables $L$ and $U$ can be computed in $O(m 2^{\sigma})$ time.
	% , where $m$ is the number of transitions in $\mathcal{A}(R)$.
	% Observe that  $m \leq n$, and hence $L$ and $U$ can be constructed in $O(m 2^{\sigma})$ time. 
	As the maximum universality of any word accepted by $\mathcal{A}$ will be equal to $\max_{q_f \in F} U[q_f, \emptyset]$, once $U$ has been computed, $k$-ESU can be determined for$\mathcal{A}$ in constant time, giving the proof.\qed
\end{proof}

==> results.tex <==
%\todoah{the following section belongs to the regular expression paper}
%{\color{orange}
%\paragraph*{Regular Expressions and Union-Free Subregular Languages}
%
%\begin{proposition}
%	Given a regular language $L\subseteq\Sigma^{\ast}$ as regular expression $r\in(\Sigma\cup\{(,),|,\ast\})^{\ast}$, we can determine the universality indices of $L$'s shortest words in time $\mathcal{O}(|r|)$.
%\end{proposition}
%
%\begin{proof}
%	First, we determine $L$'s shortest words from $r$ by deleting all Kleene parts of $r$. 
%	We maintain a stack $S$, and word $r'$ initialy set to the empty word $\varepsilon$.
%	We read $r$ from left to right.
%	Let $i\in[\vert r \vert ]$. If $S=\emptyset$ and $w[i]\in\Sigma\cup\{|\}$ then append $w[i]$ to $r'$. Whenever, we have $w[i]=($, we push $i$ on $S$. If we read $w[j]=)$, we pop the associated $($ from $S$. Thus, $r'$ does not contain the Kleene star anymore and we have $|r'|\leq|r|$ with $r'$ being of the form $r_1|r_2|\cdots|r_k$ for some $k\in\N_0$ and $r_i\in\Sigma^{\ast}$ for all $i\in[k]$. In a second step, we go over $r'$ and determine the shortest words of $L$. We have a list $\ell$, where $\ell[i]$ stores all words of length $i$ in $L(r')$: read $r'$ from left to right and for each $r_j$ copy the word into a variable $x$, count $r_j$'s letters and add $r_j$ to $\ell(|x|)$. Since the largest index of $\ell$ cannot be larger than $|r|$, we can access the smallest $i$ with $\ell[i]\neq\emptyset$. For each such $i$, we can determine $\iota(r_i)$ in time $\mathcal{O}(|r_i|)$. Since $\sum_{i\in[k],|r_i|\mbox{ min}}|r_i|\leq|r'|$, we remain in $\mathcal{O}(|r|)$.
%\end{proof}
%
%\begin{proposition}
%	Let $r$ be a regular expression describing a union-free language. Given $k \in \N$, the $k$-ESU problem can be decided in time $O(|r|)$.
%\end{proposition}
%\begin{proof}
%	Since $r$ does not contain a union operator, its universality depends on the outermost star. Let $\Sigma'$ be the alphabet of the expression within the outermost star operator that can be determined in $O(|r|)$ time. If $\Sigma' = \Sigma$ then $k$-ESU can be decided positively for all $k \in \N$. Otherwise, negatively.
%\end{proof}
%}
\todoah{$\downarrow$ I don't know what to do with this section, by the inclusion we immediately get the NP-hardness, keep is anyways because of the structural insights? if yes, where?}
\subsubsection{Ordered Languages}

% \todofda{Only holds for acyclic langauges}
%\begin{proposition}
%	We can determine if the ordered language $L$ given by an $n$-state DFA $\mathcal{A}$ is $k$-ESU, for every $k \in \mathbb{N}$ in $O(\sigma n)$ time.
%\end{proposition}
%\begin{proof}
%	Observe that $L$ is $k$-ESU if and only if there exists at least one accepting state with a self-loop labelled by each of the symbols in $\Sigma$. As we can determine if such a state exists by examination of the transition table, we can solve this problem in $O(\sigma n)$ time.\qed
%%
%	% Now, let us assume that no such state exists. Then, to determine the maximum value $k$ such that there exists at least one word with a universality of $k$, we observe that 
%%
%%	First, observe that the maximium number of transitions in $\mathcal{A}$ is $\sigma n$. 
%%	We note that 
%%
%%	Let $n = \mathcal A$. The maximal number of transitions in $\mathcal A$ is $\sigma \sum_{i=i}^{n-1}i$. Using BFS we can find all paths from an initial to a final state in runtime $O(n + \sigma \sum_{i=i}^{n-1}i)$ while computing the arch factorisation of each path in linear time in the path length. Check whether one of the final states has a self-transition with $\Sigma$ if not then answer the $k$-ESU problem negatively. Otherwise, let $F_\circ$ be this set of final states that have a self-transition with $\Sigma$ and $\ell$ be the smallest universality index amongst all paths ending in $F_\circ$. %The $k$-ESU problem can be answered positively for all $k \geq \ell$, and the $k$-USU problem can be answered positively iff $\ell =0$.
%\end{proof}

% Only if the langauge is acyclic
%\begin{theorem}
%	We can solve $k$-USU for ordered languages in time equal that of performing a depth-first search over every path in $\mathcal{A}$ starting at $q_0$.
%\end{theorem}
%\begin{proof}
%	We may assume that the path $\pi_w$ corresponding to the word $w$ with the smallest universality among any word accepted by $\mathcal{A}$ does not contain any self-loops. Therefore, we may construct the automaton $\mathcal{A}'$ from $\mathcal{A}$ by removing each self-loop from $\mathcal{A}$.\qed
%\end{proof}

\begin{theorem}
	We can solve $k$-ESU for ordered languages in time at most a factor of $O(\sigma)$ greater than that of performing a depth-first search over every path in $\mathcal{A}$ starting at $q_0$.
\end{theorem}

\begin{proof}
	We  do this by constructing an auxiliary automaton $\mathcal{A}'$ by replacing each state $q$ containing the self-loop labelled by $x_1, x_2, \dots, x_{y}$  with $2 y$ new states $q_{1}, q_2, \dots, q_{2y}$ such there is exactly one outgoing transition from each of $q_{1}, q_{2}, \dots, q_{2 y - 1}$, with the transition from $q_{i}$ labelled by $x_{i \bmod y}$ and $\delta(q_i, x_{i \bmod y}) = q_{i + 1}$. Further, for every $x \in \Sigma$ such that $\delta(q, x) = p$ where $p \neq q$, we add an outgoing transition from $q_{2 y}$ to $p$, or $p_1$, if $p$ is replaced in the same way. In doing so, note that any path $\pi_w$ ending at $q_{2y}$ will end with the suffix $x_1 x_2 \dots x_{y} x_1 x_2 \dots x_{y}$, and therefore, $x_i \in \al(\r(w)), \forall i \in [y]$. Further, as we now have an acyclic graph with at most $O(\sigma)$ more states than the original automaton, the complexity of performing a depth-first search over every path in $\mathcal{A}'$ is at most a factor of $\sigma$ more than the complexity of performing a depth-first search over every path in $\mathcal{A}$. Thus, by Lemma \ref{lem:acyclic}, we get the statement.\qed
\end{proof}\todo[inline]{I assume $x_1...x_y$ should be pairwise different but are allowed to occur more than once in the loop. Otherwise the new paths can be longer than $O(\sigma)$. Further, I don't see where we use the property "ordered" and so we should be able to transfer the result to general DFA which contradicts the NP-hardness from regular languages.}
\todoah{I think that it only suffices in ordered languages to only enroll the selfloops once. The loop structure is more complicatee for DFA}
%
%\paragraph*{Power-Separating}
%
%
%A language is power-separating if and only if, there is a natural number $m\geq 1$ such that
%for any word~$x\in V^*$, either
%$J_x^m \cap L = \emptyset$
%or
%$J_x^m\subseteq L$
%where
%$J_x^m =  \{x^n \mid n\geq m\}$,
%
%\begin{lemma}
%    Let $x \in \Sigma^*$ be a word such that $J_x^{m} \subseteq \mathcal{L}$ where $\mathcal{L}$ is a power separating language. Then, for any primitive $v$ and integer $k$ such that $v^k = x$, $J_x^{m} \subseteq \mathcal{L}$.
%\end{lemma}
%
%\begin{proof}
%    Observe that as $J_x^{m} \subseteq \mathcal{L}$, we have that $v^{m k} \in \mathcal{L}$, and thus $J_v^{m} \cap \mathcal{L} \neq \emptyset$. Therefore, either $J_x^{m}\cap \mathcal{L} = \emptyset$, contradicting the initial assumption, or $J_v^{m} \subseteq \mathcal{L}$.
%\end{proof}

%\todoah{NP-membership missing, I think this can be done by non-det. guess the integer $m$ for the language and verify that every power loops in a final state from there on?}
%\todoah{this NP-hardness updated (for the case that the graph has many hamiltonian subgraphs)}
%{\color{orange}
%\begin{proposition}
%	For a power-separating language $L$, represented by a power-separating automaton and $k \in \N$ it is NP-hard to decide the $k$-ESU problem.
%\end{proposition}
%\begin{proof}
%	We extend the idea of \cite{regunivpaper}, i.e., we are reducing from the Hamilton cycle problem. As an instance for the Hamiltonian cycle problem, we are given a graph $G = (V,E)$ with $V = \{v_1, \ldots, v_n\}$. We construct an automaton $\mathcal{A}$ containing $n^2+2$ states $Q = \{q_0, q_f\} \cup \bigcup_{i,j \in [n]} \{q_{i,j}\}$ where $q_0$ is the initial state and $q_f$ will be used as a failure state. The transition function $\delta : Q \times \Sigma \to Q$ is defined by
%	\[
%	\delta(q,k) = \begin{cases}
%		q_{1,k}, & \text{if } q = q_0,\\
%%		q_{f}, & \text{if } q = q_0 \land a \neq k,\\
%		q_{i+1,k}, & \text{if } q = q_{i,j} \land (j,k) \in G,\\
%		q_0 & \text{if } q = q_{n,j} \text{ for } j \in [n] \land k = \varepsilon, \\
%		q_{f}, & \text{otherwise.}
%	\end{cases}
%	\]
%	\todo{unsure about the loop from the final state to the initial state}
%	To give an intuition for the idea, we represent the visit of $v_j$ at the \nth{$i$} step by $q_{i,j}$.
%	Further, set $F = \{q_{n,j} \mid j \in [n]\}$. We are now showing that there exists a Hamilton cycle in $G$ if and only if the language $L(\mathcal{A})$ is a power-separating regular language such that there exists a $k$-universal word for every $k \in \N$ w.r.t.~$\Sigma = [n]_0$.
%	
%	For the first direction, assume that there exists a Hamiltonian path $p=(v_1,\ldots, v_n)$ in $G$. By construction the automaton $\mathcal{A}$ that is constructed recognises the language $u^*$ where $u$ is a permutation of $1 \cdots n$ which is a power-separating regular language containing a $k$-universal word for every $k \in \N$.
%	
%	For the second direction, assume that there does not exist a Hamilton path. Thus, by construction for any Hamiltonian path $p$ there exists a vertex that is not included, i.e., there exists at least one state $q_i \in Q$ with $q_i \notin p$. Thus, there exists some $x \in (\Sigma\setminus \{i\})^*$ such that the recognised language of $\mathcal A$ is $x^*$. Since $\al(x) \neq \Sigma$, there does not exist any $k \in \N$ together with a $w \in L(\mathcal{A})$ such that $w$ is $k$-universal, i.e., $\mathcal{A}$ and $k$ are a negative instance of $k$-ESU.
%\end{proof}}


    

% Things to prove (if possible) None work at the moment, but keeping it in for now basically as goals

% \begin{definition}[Simple Parkih Vectors]
%     Given a langauge $\mathcal{L}$ defined by the automaton $\mathcal{A}$, a Parkih vector $P$ is a \emph{simple Parkih vector} in $\mathcal{L}$ if there exists some word $w$ with the Parikh vector $P$ such that the path induced in $\mathcal{A}$ by following the transitions labelled by $w$ in order is simple (loop free).
% \end{definition}

% We denote by $SP(\mathcal{L})$ the set of simple Parkih vectors in $\mathcal{L}$

% \begin{lemma}
%    Given a permutation langauge $\mathcal{L}$ defined by the automaton $\mathcal{A}$, if there exists in $\mathcal{A}$ any state $q$ with a self loop labeled by the symbol $a \in \Sigma$, then every state has a self loop labelled by $a$, assuming the automaton is compact (does not have redundent states/paths etc.)
%\end{lemma}

%\begin{proof}
%    Assume the contradiction. Let $q$ be a state without the self loop, let $q'$ be a state with such a loop, and let $a$ be the symbol on the loop. Then, any word may contain an infinite number of occurences of the letter $a$. As the langauge is a permutation langauge, there must either be a minimum number of $a$'s needed in some words.
%\end{proof}

%\begin{lemma}
%    Given a permutation langauge $\mathcal{L}$ defined by the automaton $\mathcal{A}$, and a simple Parikh vector $P \in SP(\mathcal{L})$, any word $w$ with the Parikh vector $P$ induces a simple path in $\mathcal{L}$.
%\end{lemma}

%\begin{proof}
%    Assume the contradiction, let $w$ be some word in $\mathcal{L}$ with the Parikh vector $P$ s.t. $w$ induces a simple path in $\mathcal{A}$, and let $v$ be some word that does not induce a simple path in $\mathcal{A}$. Then, there must exist some pair $a b \in \Sigma$ such that $ab$ is a factor in $v$ but not $w$, and there exists some state with a self loop labelled by $b$. Note that if there is any state with a self loop labelled by $b$, then every state can be written with such a self loop. Therefore, the path induced 
%\end{proof}

%\begin{lemma}
%    Given a permutation langauge $\mathcal{L}$ defined by the automaton $\mathcal{A}$ with $n$ states where the Parkih vector $P \in SP(\mathcal{L})$ satisfies $\forall P' \in SP(\mathcal{L})$, $\min(i \in P') \leq \min(i \in P)$. Then, $n \geq {m \choose P[1], P[2], \dots, P[\sigma]}$, where $m = P[1] + P[2] + \dots + P[\sigma]$.
%\end{lemma}

%\begin{proof}
%    Observe that, for $\mathcal{A}$ to be a permutation langauge, there must exist a path in $\mathcal{A}$ 
% \end{proof}

%\begin{proof}
%    Let $w$ be the longest word in $\mathcal{L}$ such that the path induced in $\mathcal{A}$ formed by starting at the initial state $q_0$ and following the edges labelled by $w$ in order is simple (loop-free). Note that any (simple) path in $\mathcal{A}$ can have length at most $m = \vert w \vert$. Now, as $\mathcal{L}$ is a permutation language, we have that 
%\end{proof}

% --------------------------------------------------------------
% Works below here. All just sketches at the moment, got distracted trying to prove some relationship between m and n that makes this look nice. (above)



%\begin{lemma}
%    Given a permutation language $\mathcal{L}$ defined by the automaton $\mathcal{A}$ with $n$ states, we can determine if the universality of $\mathcal{L}$ is finite in $O(m)$ time, where $m$ is the length of the longest path in the automaton.
%\end{lemma}
%
%\begin{proof}
%    {\color{red} Informal, need to tidy up later.}
%    Start at the initial state. Follow the path induced by the first symbol $a$ until we reach a state with a self loop for $a$. Continue from here on the path induced by the second symbol $b$ until reaching a state with a self loop on $b$. Repeat for each symbol. If we reach a state with a self loop labelled by the last symbol $\sigma$, then we have infinite universality. Otherwise we do not.
%\end{proof}
%
%\begin{lemma}
%    Given a permutation language $\mathcal{L}$ defined by the automaton $\mathcal{A}$ with $n$ states, the universality of $\mathcal{L}$ can be determined in $O(m^2)$ time.
%\end{lemma}
%
%\begin{proof}
%    {\color{red} Informal, need to tidy up later.}
%    For a given $k$ universality (and I came up with this as writing the top part so it is a bit messy), we can do the same basic thing, following a path with $k$ copies of the first symbol, then moving to the first branch with a $b$ and repeating. In this case, to find the largest such $k$, we can do this in increasing order, until we find the largest value. As this can correspond to a path of length at most $k \sigma \leq m$, we get that this will take, at most $O(m^2)$ steps.
%\end{proof}

